Transport of Algebraic Structure to Latent Embeddings

Machine learning often aims to produce latent embeddings of inputs which lie in a larger, abstract mathematical space. For example, in the field of 3D modeling, subsets of Euclidean space can be embedded as vectors using implicit neural representations. Such subsets also have a natural algebraic structure including operations (e.g., union) and corresponding laws (e.g., associativity). How can we learn to "union" two sets using only their latent embeddings while respecting associativity? We propose a general procedure for parameterizing latent space operations that are provably consistent with the laws on the input space. This is achieved by learning a bijection from the latent space to a carefully designed mirrored algebra which is constructed on Euclidean space in accordance with desired laws. We evaluate these structural transport nets for a range of mirrored algebras against baselines that operate directly on the latent space. Our experiments provide strong evidence that respecting the underlying algebraic structure of the input space is key for learning accurate and self-consistent operations.

==> main-pratenddefaultcategory.tex <==


\subsection {Proofs for \cref {sec: method}} \label {app: method}

\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Let $f\in \F $, let $n = \ar (f)$, and consider the realization $f^{\M }$ on $M$ and the realization $f^{\L }$ on $L$ induced by \eqref {eq: induced_operation}. Let $z_1,\dots ,z_n\in L$. We have that \begin {align*} \iso (f^{\L }(z_1,\dots ,z_n)) &= \iso (\iso ^{-1}(f^{\M }(\iso (z_1),\dots ,\iso (z_n)))) \\ &= f^{\M }(\iso (z_1),\dots ,\iso (z_n)) \end {align*} by construction of the operation $f^\L $. Hence, we see that $\iso $ is an isomorphism from the induced algebra $\L $ to the algebra $\M $.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}Let $\iso \colon L\to M$ be a bijection, and let $\L $ be the induced latent algebra defined by \eqref {eq: induced_operation}. Let $R$ be a law that is satisfied by $\S $ (and hence satisfied by $\M $), given by \begin {equation*} p(x_1,\dots ,x_n) = q(x_1,\dots ,x_n). \end {equation*} By \cref {prop: isomorphism}, $\iso $ is an isomorphism from $\L $ to $\M $. Let $f\in \F $ be an arbitrary operation symbol. Then, by the properties of isomorphisms, it must be that \begin {equation*} \iso (f^{\L }(z_1,\dots ,z_n)) = f^{\M }(\iso (z_1),\dots ,\iso (z_n)) \end {equation*} for all $z_1,\dots ,z_n\in L$. Thus, it holds that \begin {equation*} \iso (p^{\L }(z_1,\dots ,z_n)) = p^{\M }(\iso (z_1),\dots ,\iso (z_n)) \end {equation*} for all $z_1,\dots ,z_n\in L$, and similarly, \begin {equation*} \iso (q^{\L }(z_1,\dots ,z_n)) = q^{\M }(\iso (z_1),\dots ,\iso (z_n)) \end {equation*} for all such $z_1,\dots ,z_n$. Therefore, since $\M $ satisfies the law $R$, we conclude that \begin {equation*} \iso (p^{\L }(z_1,\dots ,z_n)) = \iso (q^{\L }(z_1,\dots ,z_n)) \end {equation*} for all $z_1,\dots ,z_n\in L$. Hence, by invertibility of $\iso $, we also find that \begin {equation*} p^{\L }(z_1,\dots ,z_n) = q^{\L }(z_1,\dots ,z_n) \end {equation*} for all $z_1,\dots ,z_n\in L$, and therefore $\L $ satisfies the law $R$.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}We prove the claim by construction. Consider the source algebra $\S = (\R ,\thickcdot )$, with a sole binary operation $\thickcdot $ defined by \begin {equation*} s_1 \thickcdot s_2 = |s_1| s_2, \end {equation*} where, of course, $|s_1|$ represents the absolute value of the real number $s_1$, and $|s_1| s_2$ represents the usual product of the two real numbers $|s_1|$ and $s_2$. This source algebra is a semigroup, namely, $\R $ is closed under the binary operation $\thickcdot $, and $\thickcdot $ satisfies the associativity law, since \begin {align*} s_1\thickcdot (s_2\thickcdot s_3) &= |s_1|(s_2\thickcdot s_3) \\ &= |s_1| (|s_2|s_3) \\ &= |s_1 s_2|s_3 \\ &= \big | |s_1| s_2 \big | s_3 \\ &= (|s_1|s_2)\thickcdot s_3 \\ &= (s_1\thickcdot s_2)\thickcdot s_3 \end {align*} for all $s_1,s_2,s_3\in \R $. Now, consider the mirrored algebra $\M = (\R ,+)$, with $+$ being the standard addition operation on the real numbers. Obviously, $\M $ is also a semigroup, since $\R $ is closed under $+$, and $+$ is associative. \par We now show that $\M $ satisfies every law $R$ that $\S $ does. Let $R$ be a law for type $\F $ defined by \begin {equation*} R : p(x_1,\dots ,x_n) = q(x_1,\dots ,x_n) \end {equation*} for some arbitrary terms $p(x_1,\dots ,x_n), q(x_1,\dots ,x_n)\in T_{\F }(X)$. Suppose that $\S $ satisfies the law $R$. Then, \begin {equation*} p^{\S }(s_1,\dots ,s_n) = q^{\S }(s_1,\dots ,s_n) \end {equation*} for all $s_i\in \R $. Since the associative binary operation $\thickcdot $ is the only operation in $\F ^{\S }$, it must be that the term function $p^{\S }$ is given by some repeated application of $\thickcdot $: \begin {equation*} p^{\S }(s_1,\dots ,s_n) = s_{i_1}\thickcdot s_{i_2} \thickcdot \cdots \thickcdot s_{i_{m_p}} \end {equation*} for some $m_p\in \N $ and some tuple $(i_1,\dots ,i_{m_p})\in \{1,\dots ,n\}^{m_p}$. Similarly, \begin {equation*} q^{\S }(s_1,\dots ,s_n) = s_{j_1}\thickcdot s_{j_2} \thickcdot \cdots \thickcdot s_{j_{m_q}} \end {equation*} for some $m_q\in \N $ and some tuple $(j_1,\dots ,j_{m_p})\in \{1,\dots ,n\}^{m_p}$. Thus, \begin {equation} |s_{i_1} \cdots s_{i_{m_p}-1} | s_{i_{m_p}} = |s_{j_1} \cdots s_{j_{m_q}-1} | s_{j_{m_q}}. \label {eq: semigroup_law} \end {equation} If $m_p > m_q$, then there exists some factor $s_i$ appearing in the product $|s_{i_1}\cdots s_{i_{m_p}-1}| s_{i_{m_p}}$ at least once more than it does in the product $|s_{j_1}\cdots s_{j_{m_q}-1}| s_{j_{m_q}}$. Thus, if the equality \eqref {eq: semigroup_law} holds for some $s_1,\dots ,s_n\in S$, doubling this particular value $s_i$ would result in the law being violated, as the left-hand side of \eqref {eq: semigroup_law} would have an extra factor of $2$ that the right-hand side would not. This implies that $m_p \le m_q$. Analogous reasoning shows that $m_q \le m_p$, and hence it must be that $m_p = m_q$; the same number of factors appear in the left-hand and right-hand sides of the law's realizations. Furthermore, the same reasoning goes to show that the left-hand and right-hand products in \eqref {eq: semigroup_law} actually must contain exactly the same factors with the same multiplicity (albeit in possibly different order), i.e., the ordered tuple $(s_{i_1},\dots ,s_{i_{m_p}})$ of real numbers is some permutation of the ordered tuple $(s_{j_1},\dots ,s_{j_{m_q}})$. Hence, it must be the case that \begin {equation*} s_{i_1} + s_{i_2} + \cdots + s_{i_{m_p}} = s_{j_1} + s_{j_2} + \cdots + s_{j_{m_q}}, \end {equation*} implying that \begin {equation*} p^{\M }(s_1,\dots ,s_n) = p^{\M }(s_1,\dots ,s_n). \end {equation*} That is, the law is satisfied by $\M $ as well. Since $R$ was arbitrarily chosen, we conclude that indeed $\M $ satisfies every law $R$ that $\S $ does. \par \par \par \par \par Now, let $\psi \colon S \to M$ be a homomorphism from $\S $ to $\M $. Then, it holds that \begin {equation*} \psi (s_1\thickcdot s_2) = \psi (s_1) + \psi (s_2) \end {equation*} for all $s_1,s_2 \in S = \R $. Therefore, for $s_1=0$ and $s_2 = s$ with $s\in S$ arbitrary, we conclude that \begin {equation*} \psi (0) = \psi (|0|s) = \psi (0 \thickcdot s) = \psi (0) + \psi (s), \end {equation*} and hence \begin {equation*} \psi (0) + \psi (s) = \psi (0) + \psi (t) \end {equation*} for all $s,t\in S$. However, since $+$ is the standard addition operation on $\R $, this is only possible if \begin {equation*} \psi (s) = \psi (t) \end {equation*} for all $s,t\in S$, meaning the homomorphism $\psi $ must be the trivial mapping $\psi \colon s\mapsto C$ with $C = \psi (0)$. \par Now, let $\iso \colon L\to M$ be an arbitrary bijection. Equip $L$ with the algebra $\L $ induced by $\M $, as defined by \eqref {eq: induced_operation}. Let $\chi \colon S \to L$ be a homomorphism from $\S $ to $\L $. Then, since $\iso $ is an isomorphism from $\L $ to $\M $ (per \cref {prop: isomorphism}), the composition $\iso \circ \chi $ is a homomorphism from $\S $ to $\M $. Therefore, by our analysis above, $\iso \circ \chi $ must be a trivial homomorphism given by $\iso \circ \chi \colon s \mapsto C$ with $C = \iso \circ \chi (0)$. Hence, for all $s\in S$, we conclude that \begin {equation*} \chi (s) = \iso ^{-1}(C), \end {equation*} implying that $\chi $ must be a trivial homomorphism from $\S $ to $\L $. This concludes the proof.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Suppose that $E$ is bijective and that there exists a mirrored algebra $\M = (M,\F ^{\M })$ with $M=\Rl $ and an isomorphism $\psi \colon S\to M$. Define $\iso \colon L\to M$ by $\iso (z) = \psi \circ E^{-1}(z)$, which is well-defined since $E$ is bijective. Then, it holds that \begin {equation*} \iso \circ E(s) = \psi (E^{-1}(E(s))) = \psi (s) \end {equation*} for all $s\in S$, which proves the result.\end{proof}

\clearpage \subsection {Proofs for \cref {sec: set_case_study}} \label {app: impossibility} \paragraph {Continuity of complementation.} We briefly explain why we only consider continuous operations on the mirrored space to represent the complementation operation $\lnot $ in the Boolean lattice type $\FB $. Consider the complementation operation ${}^c: \pow (\Rd ) \to \pow (\Rd )$. As there is no ambient topology on $\pow (\Rd )$, the continuity of ${}^c$ is not well-defined in this context. However, a natural topology arises by passing first to the Borel sets $\Sigma $ on $\Rd $ and then quotienting by the null ideal $\Sigma \cap \mathcal {N}$, with set intersection, union, and complementation inherited in the natural way. Following \citet [323A.iii.e]{fremlin2000measure}, this allows us to define a topology via the \emph {symmetric difference metric}: \begin {equation*} d(A, B) \coloneqq \mu (A \triangle B) ~ \text {for all $A, B \in \Sigma / \Sigma \cap \mathcal {N}$}, \end {equation*} where $\mu $ is inherited naturally on the quotiented space from the Borel measure on $\Rd $. Since the symmetric difference between $A$ and $B$ satisfies $A \triangle B = (A^c) \triangle (B^c)$, it is immediate that the inherited complementation operation is continuous with respect to this topology. \par \paragraph {Negative result.} Before proving our main result, we first present a key result from the algebraic topology literature. \begin {proposition} \label {prop: fixedpoint} Any continuous involution on $\R ^n$ has a fixed point. \end {proposition} \begin {proof}[Proof of \cref {prop: fixedpoint}] This is an easy application of Theorem 9 in \citet {jaworowski1956antipodal}. Namely, $\R ^n$ is a separable metric space, and it is acyclic because it is contractible. \end {proof} \par \begin {lemma} \label {lem: lnot_involution} Consider a Boolean lattice $\A = (A,\land ,\lor ,\lnot ,0,1)$ of type $\FB $ and its associated laws in \cref {tab: lattice_laws}. Then, it holds that $\lnot $ is an involution with no fixed points. \end {lemma} \begin {proof}[Proof of \cref {lem: lnot_involution}] Clearly, the Boolean lattice laws in \cref {tab: lattice_laws} imply that $\lnot (\lnot a) = a$ for all $a\in A$, and thus $\lnot $ is an involution. Now assume for the sake of contradiction that $\lnot $ has a fixed point $b\in A$, so that $\lnot b = b$. Then, by the Boolean lattice laws, \begin {equation*} (\lnot b) \land b = 0 \implies b \land b = 0 \implies b = 0, \end {equation*} and, similarly, \begin {equation*} (\lnot b) \lor b = 1 \implies b \lor b = 1 \implies b = 1. \end {equation*} This is a contradiction. \end {proof} \par We are now ready to prove a general negative result.

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Suppose for the sake of contradiction that there exists an algebra $\B =(B,\F ^{\B })$ on $B = \Rl $ such that $\smallsquare ^{\B }$ is continuous and the laws $R_1,\dots ,R_n$ are all satisfied by $\B $. Then, by assumption it must be the case that $\smallsquare ^{\B }(b) \ne b$ for all $b\in B$. However, since $\smallsquare ^{\B }$ is a continuous involution on $B = \Rl $, by \cref {prop: fixedpoint}, $\smallsquare ^{\B }$ has a fixed point, i.e., $\smallsquare ^{\B }(b) = b$ for some $b\in B$. This is a contradiction, and hence the result is proven.\end{proof}

\prAtEndRestatevii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}This follows directly from \cref {lem: lnot_involution} and \cref {thm: no_fixedpoint_involution}.\end{proof}

